Clues on the Origin and Evolution of Massive Contact Binaries: Atmosphere Analysis of VFTS 352

The massive O4.5 V + O5.5 V binary VFTS 352 in the Tarantula nebula is one of the shortest-period and most massive overcontact binaries known. Recent theoretical studies indicate that some of these systems could ultimately lead to the formation of gravitational waves via black hole binary mergers through the chemically homogeneous evolution pathway. By analyzing ultraviolet-optical phase-resolved spectroscopic data, we aim to constrain atmospheric and wind properties that could be later used to confront theoretical predictions from binary evolution. In particular, surface abundances are powerful diagnostics of the evolutionary status, mass transfer and the internal mixing processes. From a set of 32 VLT/FLAMES visual and 8 HST/COS ultraviolet spectra, we used spectral disentangling to separate the primary and secondary components. Using a genetic algorithm wrapped around the NLTE model atmosphere and spectral synthesis code FASTWIND, we perform an 11-parameter optimization to derive the atmospheric and wind parameters of both components, including the surface abundances of He, C, N, O and Si. We find that both components are hotter than expected compared to single-star evolutionary models indicating that additional mixing processes may be at play. However the derived chemical abundances do not show significant indications of mixing when adopting baseline values typical for the system environment.

==> binary_subsection10_revised.tex <==


Since there is no suitable grid of binary models available (see however \citealt{marchant2016}), we computed a set of binary-star models by varying initial periods (P=1.0-1.2\,days) and masses ($q=M_{2}/M_{1}=0.6-1$ and $M_{2}+M_{1}=56.4\,\mathrm{M}_{\odot}$, the currently-inferred total mass of the system), and assuming a rotational mixing factor of $f_\mathrm{c}$=0.033, which is a commonly adopted value \citep{heger2000}. At the start of the calculation the stars begin with a uniform initial composition, one taken as appropriate for young stars in the LMC by \citet{brott2011}. For these calculations we used the stellar evolution package MESA (version 10398, \citealt{paxton2011,paxton2013,paxton2015,paxton2018}), with the physical assumptions from \citet{marchant2016} for modelling the over-contact phase. Mass transfer is treated as conservative. The parameters used to compute our models are available as MESA inlist files \footnote{\url{https://github.com/orlox/mesa_input_data/tree/master/2016_double_bh}}.

We find the best-fit binary model from our grid to be an equal-mass binary, with initial masses of $28.74+28.74\,\mathrm{M}_{\odot}$ and an orbital period of 1.07\,days. This system is initially in an over-contact configuration (i.e., both stars are larger than their Roche lobes), and it soon detaches and then once again reaches overcontact as the stars expand on the main sequence. There is no net mass transfer in this system since the stars begin with equal masses. The stars are in an over-contact configuration on the main sequence at $\approx1.8\,$Myr, at which stage this model has stellar masses, radii, rotational velocities, a mass ratio, and an orbital period that are roughly consistent with the observationally-inferred parameters. It does not, however, reproduce the observed luminosities or effective temperatures.  This calculation continues until the stars overflow their outer Lagrangian points, after which a merger can be expected to take place.  

We also tested an enhanced-mixing version of this model, keeping all other initial parameters the same and only changing the rotational mixing factor to $f_\mathrm{c} = 0.2$.  This model again predicts luminosities and temperatures lower than the observationally-inferred values for VFTS 352.  This may indicate more efficient mixing of helium in this system than in our models. 


========

The following is for the response:

REVIEWER'S COMMENTS:

Experiments with the MESA star models should be explained
in more detail. Was the initial binary already an over-contact system?
Was there mass transfer? Just conservative? Uniqueness of such
attempts at the present art of modeling is not guaranteed, I am
afraid.

RESPONSE:

We certainly agree with the referee that this set of models is not the only possible set of relevant models, and does not represent a uniquely viable set of assumptions or calculations.   We state in the conclusions section that this is only a preliminary investigation, and we never intended to suggest that we were presenting the only possible models here.  In a separate paper dedicated to contact systems we intend to explore a larger range of plausible physical parameters to investigate to what extent the modelling can be constrained by observed systems. 

We also accept that it would be good to provide more details of these calculations.  We now state more of our assumptions, and also indicate where the interested reader can find the exact set of physical parameters we used. In the initial version we perhaps went too far in trying to be concise.   We also now include the initial parameter range used for the exploratory study.

The calculation in our equal-mass best-fit model started in an overcontact configuration, when the binary contained uniform-composition stellar models, then broke contact, and once more reached contact as the stars expanded on the main sequence.   Since that model contains identical-mass stars, mass isn't transferred.  However, when mass transfer occurred in our exploratory grid we assumed it to be conservative.  We have now stated this explicitly in the text, as we should have done originally.  

